hp3D User Manual

User Manual for the hp3D Finite Element Software, available on GitHub at https://github.com/Oden-EAG/hp3d

==> Chapters/1_INTRODUCTION/comments.tex <==
\section*{Historical Comments}



==> Chapters/2_INSTALLING/comments.tex <==
\section*{Historical Comments}



==> Chapters/3_BASICS/comments.tex <==
\section*{Historical Comments}



==> Chapters/4_ADVANCED/comments.tex <==
\section*{Historical Comments}



==> Chapters/5_PARALLEL/comments.tex <==
\section*{Historical Comments}


